Model merging with SVD to tie the Knots

Recent model merging methods demonstrate that the parameters of fully-finetuned models specializing in distinct tasks can be combined into one model capable of solving all tasks without retraining. Yet, this success does not transfer well when merging LoRA finetuned models. We study this phenomenon and observe that the weights of LoRA finetuned models showcase a lower degree of alignment compared to their fully-finetuned counterparts. We hypothesize that improving this alignment is key to obtaining better LoRA model merges, and propose KnOTS to address this problem. KnOTS uses the SVD to jointly transform the weights of different LoRA models into an aligned space, where existing merging methods can be applied. In addition, we introduce a new benchmark that explicitly evaluates whether merged models are general models. Notably, KnOTS consistently improves LoRA merging by up to 4.3% across several vision and language benchmarks, including our new setting. We release our code at: https://github.com/gstoica27/KnOTS.

==> figures/scaling_figure.tex <==
\begin{wrapfigure}{r}{0.48\linewidth}
\vspace{7pt}
\centering
\includegraphics[width=\linewidth]{figures/Fig2_eraseSFalse_light.png}
% \includegraphics[width=\linewidth]{figures/scales_v5.pdf}
% \newline
% \vspace{-0.5em}
\caption{
{\bf \name{} alignment boosts performance with scale.} \name{}-TIES continues to see gains, outperforming original TIES \citep{yadav2023resolving} and Task Arithmetic (TA) \citep{ilharco2023editing} when merging an increasing number of tasks in the per-task vision setting \ref{sec:per_task}.
%{\bf \name{} merges significantly better} than using the original weights for LoRA \cite{hu2021lora} finetuned from the same pretrained model. 
%Aligning with \name{} then merging with TIES \cite{yadav2023resolving} scales significantly better as more models are merged than prior work (Task-Arithmetic \cite{ilharco2022editing} and TIES), \textit{without finetuning}.
Performance is 
% measured as 
the average normalized accuracy with 95\% confidence intervals over merging different combinations of the tasks
% each LoRA model was trained on, as defined in \citet{ilharco2023editing, yadav2023resolving}. 
% See Section \ref{sec:results} for more details.
% both task-arithmetic \cite{ilharco2022editing} and TIES \cite{yadav2023resolving} when merging
% and reporting the average normalized accuracy with 95\% CIs on per-task evaluations. [TODO: add caption]
}
\label{fig:incremental_figure}
% \end{table}
\vspace{-25pt}
\end{wrapfigure} 

==> figures/scaling_lora_rank.tex <==
\begin{wrapfigure}{r}{0.48\linewidth}
\vspace{7pt}
\centering
\includegraphics[width=\linewidth]{figures/lora_across_rank.png}
% \includegraphics[width=\linewidth]{figures/scales_v5.pdf}
% \newline
% \vspace{-0.5em}
\caption{
{\bf \name{} alignment boosts performance across LoRA ranks.} \name{}-TIES consistently outperforms TIES \citep{yadav2023resolving} across varying LoRA ranks in the per-task vision setting. Performance is reported in terms of average normalized accuracy across eight vision tasks.
}
\label{fig:scaling_lora_rank}
% \end{table}
\vspace{-25pt}
\end{wrapfigure} 
